Tree Learning: Optimal Algorithms and Sample Complexity

We study the problem of learning a hierarchical tree representation of data from labeled samples, taken from an arbitrary (and possibly adversarial) distribution. Consider a collection of data tuples labeled according to their hierarchical structure. The smallest number of such tuples required in order to be able to accurately label subsequent tuples is of interest for data collection in machine learning. We present optimal sample complexity bounds for this problem in several learning settings, including (agnostic) PAC learning and online learning. Our results are based on tight bounds of the Natarajan and Littlestone dimensions of the associated problem. The corresponding tree classifiers can be constructed efficiently in near-linear time.

==> env_defs.tex <==
\newenvironment{theorem}[1][]{%
\begin{thm1}[#1]%
}{\end{thm1}%
}
\newenvironment{lemma}[1][]{%
\begin{lem1}[#1]%
}{\end{lem1}%
}
\newenvironment{observation}[1][]{%
\begin{obs1}[#1]%
}{\end{obs1}%
}
\newenvironment{inv}[1][]{%
\begin{inv1}[#1]%
}{\end{inv1}%
}
\newenvironment{fact}[1][]{%
\begin{fact1}[#1]%
}{\end{fact1}%
}
\newenvironment{remark}[1][]{%
\begin{rem1}[#1]%
}{\end{rem1}%
}
\newenvironment{pthm}[1][]{%
\begin{pthm1}[#1]%
}{\end{pthm1}%
}
\newenvironment{corollary}[1][]{%
\begin{cor1}[#1]%
}{\end{cor1}%
}
\newenvironment{definition}[1][]{%
\begin{defn1}[#1]%
}{\end{defn1}%
}
\newenvironment{asmp}[1][]{%
\begin{asmp1}[#1]%
}{\end{asmp1}%
}
\newenvironment{proposition}[1][]{%
\begin{prop1}[#1]%
}{\end{prop1}
}%

\if 1\special
    \if 1\highlight
        \renewenvironment{theorem}[1][]{%
        \begin{mdframed}[nobreak=false,backgroundcolor=Aquamarine!60]\begin{thm1}[#1]%
        }{\end{thm1}\end{mdframed}%
        }
        \renewenvironment{lemma}[1][]{%
        \begin{mdframed}[nobreak=false,backgroundcolor=YellowGreen!60]\begin{lem1}[#1]%
        }{\end{lem1}\end{mdframed}%
        }
        \renewenvironment{observation}[1][]{%
        \begin{mdframed}[nobreak=false,backgroundcolor=Salmon!60]\begin{obs1}[#1]%
        }{\end{obs1}\end{mdframed}%
        }
        \renewenvironment{inv}[1][]{%
        \begin{mdframed}[nobreak=false,backgroundcolor=Salmon!60]\begin{inv1}[#1]%
        }{\end{inv1}\end{mdframed}%
        }
        \renewenvironment{fact}[1][]{%
        \begin{mdframed}[nobreak=false,backgroundcolor=Salmon!60]\begin{fact1}[#1]%
        }{\end{fact1}\end{mdframed}%
        }
        \renewenvironment{pthm}[1][]{%
        \begin{mdframed}[nobreak=false,backgroundcolor=Salmon!60]\begin{pthm1}[#1]%
        }{\end{pthm1}\end{mdframed}%
        }
        \renewenvironment{proposition}[1][]{%
        \begin{mdframed}[backgroundcolor=Goldenrod!60]\begin{prop1}[#1]%
        }{\end{prop1}\end{mdframed}%
        }
        \renewenvironment{asmp}[1][]{%
        \begin{mdframed}[backgroundcolor=Goldenrod!60]\begin{asmp1}[#1]%
        }{\end{asmp1}\end{mdframed}%
        }
        \renewenvironment{corollary}[1][]{%
        \begin{mdframed}[backgroundcolor=Mulberry!60]\begin{cor1}[#1]%
        }{\end{cor1}\end{mdframed}%
        }
    \fi
    \if 1\sidebar
        \tcolorboxenvironment{theorem}{blanker,breakable,left=4mm, before skip=10pt,after skip=10pt, borderline west={2mm}{0pt}{Aquamarine}}
        \tcolorboxenvironment{lemma}{blanker,breakable,left=4mm, before skip=10pt,after skip=10pt, borderline west={2mm}{0pt}{YellowGreen}}
        \tcolorboxenvironment{observation}{blanker,breakable,left=4mm, before skip=10pt,after skip=10pt, borderline west={2mm}{0pt}{Salmon}}
        \tcolorboxenvironment{inv}{blanker,breakable,left=4mm, before skip=10pt,after skip=10pt, borderline west={2mm}{0pt}{Salmon}}
        \tcolorboxenvironment{fact}{blanker,breakable,left=4mm, before skip=10pt,after skip=10pt, borderline west={2mm}{0pt}{Salmon}}
        \tcolorboxenvironment{pthm}{blanker,breakable,left=4mm, before skip=10pt,after skip=10pt, borderline west={2mm}{0pt}{Salmon}}
        \tcolorboxenvironment{proposition}{blanker,breakable,left=4mm, before skip=10pt,after skip=10pt, borderline west={2mm}{0pt}{Goldenrod}}
        \tcolorboxenvironment{corollary}{blanker,breakable,left=4mm, before skip=10pt,after skip=10pt, borderline west={2mm}{0pt}{Mulberry}}
        \tcolorboxenvironment{asmp}{blanker,breakable,left=4mm, before skip=10pt,after skip=10pt, borderline west={2mm}{0pt}{Goldenrod}}
    \fi
\fi

%	\expandafter\let\expandafter\oldproof\csname\string\proof\endcsname
%	\let\oldendproof\endproof
%	\renewenvironment{proof}[1][\proofname]{%
%		\begin{mdframed}[backgroundcolor=lightgray!60]\oldproof[#1]%
%		}{\oldendproof\end{mdframed}}


\if 1\specialproof
    \if 1\highlight
        \expandafter\let\expandafter\oldproof\csname\string\proof\endcsname
        \let\oldendproof\endproof
        \renewenvironment{proof}[1][\proofname]{%
        \begin{mdframed}[nobreak=false,backgroundcolor=lightgray!10]\oldproof[#1]%
        }{\oldendproof\end{mdframed}}
    \else
        \if 1\sidebar
        \tcolorboxenvironment{proof}{
        blanker,breakable,left=4mm,
        before skip=10pt,after skip=10pt,
        borderline west={2mm}{0pt}{lightgray}}
        \fi
    \fi
\fi


\if 1\specialdefinition
    \if 1\highlight
        \renewenvironment{definition}[1][]{%
        \begin{mdframed}[innerbottommargin=0.1cm,innertopmargin=0.1cm,backgroundcolor=Apricot!60]\begin{defn1}[#1]%
        }{\end{defn1}\end{mdframed}%
        }
    \else
        \if 1\sidebar
        \tcolorboxenvironment{definition}{
        blanker,breakable,left=4mm,
        before skip=10pt,after skip=10pt,
        borderline west={2mm}{0pt}{Apricot}}
        \fi
    \fi
\fi


\if 1\specialremark
    \if 1\highlight
        \renewenvironment{remark}[1][]{%
        \begin{mdframed}[backgroundcolor=Salmon!60]\begin{rem1}[#1]%
        }{\end{rem1}\end{mdframed}%
        }
    \else
        \if 1\sidebar
        \tcolorboxenvironment{remark}{
        blanker,breakable,left=4mm,
        before skip=10pt,after skip=10pt,
        borderline west={2mm}{0pt}{Salmon}}
        \fi
    \fi
\fi

\if 1\colorequations
    \everymath{\color{MidnightBlue}}
\fi


==> sections/acknowledgements.tex <==
\section*{Acknowledgements}


==> sections/near_linear_time_alg.tex <==
\section{Near-Linear Algorithm for Constructing an HCT for Triplet Constraints}
In this section, we show how to leverage our new perspective on triplet constraint satisfaction to design a very simple $O(m\log^2{n}+n\alpha(m,n))$ time algorithm for constructing an HCT consistent with a set of $m$ given triplet constraints over $n$ points.
This significantly improves the previous results of \orr{add here some related work stuff} \danny{the citation is \cite{Inferring_a_tree_from_lowest_common_ancestors_with_an_application_to_the_optimization_of_relational_expressions} - but I think this should be moved to the introduction.}

\begin{theorem}
\label{thm:htc_construction_alg}
Let $V = \{v_1,\dots,v_n\}$ be a set of points, and $\bar{\Delta} = \{(a_i|b_ic_i)\}_{i=1}^m $ a set of triplet constraints. There is a deterministic $O(m\log^2{n}+n\alpha(m,n))$ time algorithm which outputs a binary hierarchical clustering tree consistent with all constraints in $\bar{\Delta}$, or outputs that no such tree exists.
\end{theorem}

In our algorithm, we use the decremental Minimum Spanning Forest (MSF) data-structure of \cite{HLT01}:
\begin{theorem}[\cite{HLT01} Theorem 6]
\label{thm:decrement_msf}
There exists a deterministic decremental MSF data-structure that can be initialized on a graph with $n$ vertices and $m$ edges and supports any sequence of deletions in $O(m\log^2{n})$ total time.
\end{theorem} 

While we use the the data-structure of \cite{HLT01} in an almost black-box manner, we need to note a few very simple facts regarding it for our algorithm. Whenever an edge in the maintained MFS is deleted, a single replacement edge is found and added to the MSF (unless no replacement edge exists), and the rest of the forest remains unchanged. When a non-forest edge is deleted, the maintained MSF is unchanged. Whenever a deletion in the MSF occurs, the data-structure reports the replacement edge that was chosen. We can augment the data-structure to return after a deletion (a) the heaviest edge in the new MSF, (b) which (if any) vertices became isolated after the deletion, and (c) the number of connected components in the MSF in the following manner - since at most two edges are changed in the maintained MSF during a deletion, this augmentation can be trivially implemented by (a) maintaining a maximum heap on the edges of the maintained MFS, which can be done in $O(\log{n})$ time per deletion, (b) maintaining a counter for each vertex, which contains its degree, which can be done in $O(1)$ time per deletion, and (c) a counter of the number of edges in the MSF after a deletion, which is decreased by one each time a deletion of a MSF edge is performed but a replacement edge was not found. We also note that the data-structure works for multi-graphs. \orr{Move to appendix and expand}

Next, we describe our algorithm for constructing an HTC satisfying the constraints of $\bar{\Delta}$, or rejects if no such tree exists. First, we construct a weighted multi-graph $G$ on $n$ vertices and $m$ edges from $\bar{\Delta}$ in the following manner: For each $(a_i|b_ic_i)$, we add the edge $\{b_i,c_i\}$ with weight $1$, and an edge $\{a_i,b_i\}$ with weight $2$. For convenience, we call the set of edges of weight $1$ \emph{blue edges}, the edges of weight $2$ \emph{red edges}, and denote these sets $E_{\mathrm{blue}},E_{\mathrm{red}}$ respectively. For each such $\{b_i,c_i\}$ and $\{a_i,b_i\}$ added, we say that the edges are coupled and maintain a mapping $M$ that maps each $\{b_i,c_i\}$ to its coupled $\{a_i,b_i\}$.

We initialize the data-structure of Theorem~\ref{thm:decrement_msf} on $G$, which we denote by $A(G)$. At the first phase of the algorithm, we run the Cut-Inter-Component-Edges sub-procedure, detailed in the next paragraph, in iterations $j=1,\dots,...$ until either the sub-procedure rejects (in which case, we output that no HTC satisfying the constraints exists) or the graph of $A(G)$ contains only isolated nodes. We denote the $j$'th iteration of this phase by $\StepOne{j}$, and $L_j$ the list returned by the Cut-Inter-Component-Edges sub-procedure run in this iteration. Let $r$ be the number of iterations $\StepOne{1},\dots,\StepOne{r}$ of the first phase.

%\begin{tcolorbox}
\paragraph{Cut-Inter-Component-Edges sub-procedure:} First, we initialize a linked list $\mathrm{Del} = \emptyset$. Let $e_1$ be the heaviest edge in the MSF of $A(G)$ at the start of the sub-procedure. We proceed in iterations until the heaviest edge in the MSF is a blue edge. At the start of the $i$'th step, if the heaviest edge $e_i$ is a red edge, we delete $e_i$ from $A(G)$ and add its coupled edge $e'_i$  to $\mathrm{Del}$, marking it for later deletion, and to the end of the $L$. If $e_i$ is a red edge, then we instead remove the edges in $\mathrm{Del}$ marked for deletion $e'_1,\dots,e'_{i-1}$ from $A(G)$ and return the list $L=\mathrm{Del}$. This concludes the sub-procedure.
%\end{tcolorbox}

After the end of the first phase of the algorithm, we construct an HTC $T^*$ in the following manner: We initialize $T^*$ to be a collection of isolated vertices $v_1,\dots,v_n$ (one for each point), and initialize a union-find data-structure $U$ where each vertex $v_i$ is in a separate set.
For $j=r\dots,1$, where the $j$'th iteration is denoted as $\StepTwo{j}$ we perform the following: let $\{x_{1},y_{1}\},\dots,\{x_{k},y_{k}\}$ be the edges of $L_j$.
For $i=1,\dots,k$, we check whether $U$ the set of $x_{k-i}$ and the set of $y_{k-i}$ are the same. If they are not, we perform a union operation in $U$ between $x_{k-i}$ and $y_{k-i}$, add a new vertex $t_i$ to $T^*$, and connect in $T^*$ both the root of the tree containing $x_{k-i}$ and the root of the tree containing $y_{k-i}$ as children of $t_i$. 

Let $c$ be the number of trees in $T^*$ at the end of $\StepTwo{j}$, and $T_1,\dots,T_c$ the trees of $T^*$ at this time (numbered arbitrarily). If $c > 1$ we add new vertices $t'_1,\dots,t'_c$ to $T^*$, and for each $i < c$ connect in $T^*$ the vertices $t'_{i+1}$ as a child of $t'_{i}$, and the root of $T_i$ as a child of $t'_i$. Finally, we output $T^*$.



\paragraph*{Correctness:} 
\begin{lemma}
    \label{lem:alg_terminates}
    The algorithm terminates after $O(m\log^2{n}+n\alpha(m,n))$ time.
\end{lemma}
\begin{proof}
    We can bound the running time of the first phase by $O(m\log^2{n}+n)$, since we all deletion operations on $A(G)$ have a total running time of $O(m\log^2{n})$, and we otherwise perform $O(m+n)$ elementary operations for maintaining supporting data-structures such as $L$ and $\mathrm{Del}$. In the second phase, we perform at most $O(m+n)$ operations on $U$, costing us $O((m+n)\alpha(m,n)))$, as well as performing $O(m+n)$ of maintaining supporting data-structures.
\end{proof}

Before proving correctness and soundness, we recall that by Lemma~\orr{todo: ref}, if $\bar{\Delta}$ is satisfiable by an HTC if and only if for any $H'_{blue} \subseteq E_{\mathrm{blue}}$ and their coupled edges $H'_{red} \subseteq E_{\mathrm{red}}$, then for $S = V(E')$, the graph $G[S]$ does not contain a spanning tree on the blue edges. \orr{this needs a proof very similar to the one we have in the triplet part}

\begin{lemma}[Soundness]
    \label{lem:alg_soundness}
    If the algorithm rejects, then there exists no HTC which satisfies all constraints of $\bar{\Delta}$.
\end{lemma}
\begin{proof}
    Assume that the algorithm rejects, meaning that for some $j^*$, in the start of $\StepOne{j^*}$ the heaviest edge of the MSF of $A(G)$ is blue. In particular, since the graph is not a collection of isolated vertices, the blue edges in $A(G)$ at the start of $j^*$ have a connected component $S \subseteq V$ which contains more than one vertex, composed by some blue edges $\{x_1,y_1\},\dots,\{x_k,y_k\}$. 
    
    We note that for each of their coupled red edges $\{x'_1,y'_1\},\dots,\{x'_k,y'_k\}$, both $x'_i$ and $y'_i$ must be in $S$ - Otherwise, by construction, $\{x_i,y_i\}$ and $\{x'_i,y'_i\}$ share a vertex (w.l.o.g $x_i=x'_i$), and if $y'_i$ is contained in a different connect component of the blue edges, then the heaviest edge in the MSF of $A(G)$ at the start of $j^*$ must be a red edge, which is a contradiction. 
    
    Therefore, $S$ contains all endpoints of $\{x_1,y_1\},\dots,\{x_k,y_k\}$ and $\{x'_1,y'_1\},\dots,\{x'_k,y'_k\}$, and by Lemma~\orr{todo: ref} this implies that the constraints of $\bar{\Delta}$ are not satisfiable by an HTC.
\end{proof}

Before completing the proof of correctness, we prove a few useful invariants of the algorithm.

\begin{lemma}
\label{lem:step1_cc_is_step2_backwards}
    For any $1 \leq i \leq r$, At the start of $\StepTwo{i}$, the set of each vertex $v$ in $U$ is its blue edged connected component in $A(G)$ at the start of $\StepOne{r-i+1}$
\end{lemma}
\begin{proof}
     Recall that since the algorithm does not reject, $\bigcup_i L_i$ is the set of all blue edges in the initial graph $G$. For any $0 \leq i \leq r$, at steps $\StepOne{1},\dots,\StepOne{r-i+1}$ we removed $L_1,\dots,L_{r-i+1}$, meaning that the remaining blue edges are exactly $L_{r-i},\dots,L_{r}$. In $\StepTwo{1},\dots,\StepTwo{i}$, we process each blue edge $\{x_j,y_j\}$ in $L_{r-i},\dots,L_{r}$ and union the sets of $\{x_j,y_j\}$ (if they are not already in the same set), which implies that the sets in $U$ are exactly these blue connected components.
\end{proof}

\begin{lemma}
\label{lem:deleted_red_is_intercomponent}
    If a red edge $\{x,y\}$ is deleted during $\StepOne{i}$, then the vertices $x$ and $y$ do not have a path in $E_{\mathrm{blue}}$ at the start of $\StepOne{i}$.
\end{lemma}
\begin{proof}
    Recall that if $\{x,y\}$ is a red edge that is deleted during $\StepOne{i}$, then it is in the MSF of $A(G)$ at some time during $\StepOne{i}$. In addition, no blue edge is deleted between the start of $\StepOne{i}$ and that time (blue edges are only deleted near the end of a step). Therefore, there is no blue path between $a$ and $c$ at the start of $\StepOne{i}$; Otherwise, $\{x,y\}$ could be replaced by a blue edge while maintaining the same connected components, reducing the total weight of the MSF, contradiction to its minimality.
\end{proof}

\begin{lemma}[Correctness]
    \label{lem:alg_correctness}
    If the algorithm does not reject, it outputs an HTC $T^*$ satisfying all constraints of $\bar{\Delta}$.
\end{lemma}
\begin{proof}
    Assume by contradiction that some constraint $(a|bc) \in \bar{\Delta}$ is unsatisfied by $T^*$, and let $i$ such that $\{a,b\} \in L_i$. By Lemma~\ref{lem:deleted_red_is_intercomponent} the red edge $\{a,c\}$ must be an inter-component edge in the blue connected components of $\StepOne{i}$ This implies that at the start of $\StepOne{i+1}$, $a$ is in a different blue connected component than both $b,c$. By Lemma~\ref{lem:step1_cc_is_step2_backwards}, in $\StepTwo{r-i+1}$ is $b,c$ are in the same set in $U$, but $a$ is not in this set. By construction of $T^*$, this implies that $b,c$ are contained in a subtree which does not contain $a$, meaning that $(a|bc)$ is satisfied, contradiction.
\end{proof}

\subsection{Extension to $k$-constraint satisfaction}
In this subsection, we show how to extend our algorithm to a near-linear algorithm for computing an HTC for $k$-hierarchical constraints. 

\begin{theorem}
Let $V = \{v_1,\dots,v_n\}$ be a set of points, and $\bar{\Delta} = \{T_1,\dots,T_l\}_{i=1}^m $ a set of $k$-hierarchical constraints. There is a deterministic $O(mk\log^2{n}\log{k}+n\alpha(m\log{k},n))$ time algorithm which outputs a binary hierarchical clustering tree consistent with all constraints in $\bar{\Delta}$, or outputs that no such tree exists.
\end{theorem}

We reduce to the triplet constraint algorithm of Theorem~\ref{thm:htc_construction_alg}. 

\begin{lemma}[TODO:cite]
\label{lem:define_tree_by_constraints}
    For an HTC $T$ with $t$ leaves, there exists a set of triplet constraints $\{a_i|b_ic_i\}_{i=1}^{O(t\log{t}}$ such that $T$ satisfies all constraints in $\bar{\Delta}_T$, and no other tree $T'$ on $t$ leaves satisfies $\bar{\Delta}_T$. Such a set $\bar{\Delta}_T$ can be computed in $O(t\log{t}$ time.
\end{lemma}
\begin{remark}
We note that the size of the input is $O(mk\log{n}+n)$, \orr{write better}
\end{remark}

Let $\widetilde{\Delta} = \bigcup_{i=1}^l \Delta_{T_i}$, where $\Delta_{T_i}$ is a set of size $O(k\log{k}$ uniquely defining $T_i$ of Lemma~\ref{lem:define_tree_by_constraints}. We run the algorithm of Theorem~\ref{thm:htc_construction_alg} on $\widetilde{\Delta}$.

\begin{lemma}
    If the algorithm rejects, then there exists no HTC which satisfies all constraints of $\bar{\Delta}$. If the algorithm does not reject, it outputs an HTC $T^*$ satisfying all constraints of $\bar{\Delta}$.
\end{lemma}
\begin{proof}
    By Lemma~\ref{lem:define_tree_by_constraints}, for any $0 \leq i \leq l$ the constraint defined by $T_i$ is equivalent to the set of constraints $\bar{\Delta}_T$ \orr{is this clear?}. Correctness immediately follows from Lemma~\ref{lem:alg_correctness} and Lemma~\ref{lem:alg_soundness}.
\end{proof}

==> temp_commands.tex <==

\theoremstyle{plain}
\newtheorem{thm1}{Theorem}[section]
\theoremstyle{remark}
\newtheorem{pthm1}[thm1]{Theorem}
\theoremstyle{plain}
\newtheorem{lem1}[thm1]{Lemma}
\theoremstyle{plain}
\newtheorem{obs1}[thm1]{Observation}
\theoremstyle{plain}
\newtheorem{inv1}[thm1]{Invariant}
\theoremstyle{plain}
\newtheorem{cor1}[thm1]{Corollary}
\theoremstyle{definition}
\newtheorem{defn1}[thm1]{Definition}
\theoremstyle{plain}
\newtheorem{fact1}[thm1]{Fact}
\theoremstyle{remark}
\newtheorem{rem1}[thm1]{Remark}
\theoremstyle{plain}
\newtheorem{prop1}[thm1]{Proposition}
\theoremstyle{plain}
\newtheorem{asmp1}[thm1]{Assumption}

%cleveref names
% \crefname{thm1}{Theorem}{Theorems}
% \crefname{pthm1}{Theorem}{Theorems}
% \crefname{lem1}{Lemma}{Lemmas}
% \crefname{obs1}{Observation}{Observations}
% \crefname{inv1}{Invariant}{Invariants}
% \crefname{cor1}{Corollary}{Corollaries}
% \crefname{defn1}{Definition}{Definitions}
% \crefname{fact1}{Fact}{Facts}
% \crefname{rem1}{Remark}{Remarks}
% \crefname{prop1}{Proposition}{Propositions}
% \crefname{asmp1}{Assumption}{Assumptions}
% \crefname{subsection}{Subsection}{Subsections}
% \crefname{figure}{Figure}{Figures}


\ifx\proof\undefined
\newenvironment{proof}[1][\protect\proofname]{\par
\normalfont\topsep6\p@\@plus6\p@\relax
\trivlist
\itemindent\parindent
\item[\hskip\labelsep\scshape #1]\ignorespaces
}{%
\endtrivlist\@endpefalse
}
\providecommand{\proofname}{Proof}
\fi


%%%parameters for env_defs

\def\special{1}
\def\specialproof{1}
\def\specialdefinition{1}
\def\specialremark{1}
\def\highlight{1}
\def\sidebar{0}

%color all equations in some color (blue)
\def\colorequations{0}

\input{env_defs.tex}

